SkipAnalyzer: A Tool for Static Code Analysis with Large Language Models

We introduce SkipAnalyzer, a large language model (LLM)-powered tool for static code analysis. SkipAnalyzer has three components: 1) an LLM-based static bug detector that scans source code and reports specific types of bugs, 2) an LLM-based false-positive filter that can identify false-positive bugs in the results of static bug detectors (e.g., the result of step 1) to improve detection accuracy, and 3) an LLM-based patch generator that can generate patches for the detected bugs above. As a proof-of-concept, SkipAnalyzer is built on ChatGPT, which has exhibited outstanding performance in various software engineering tasks. To evaluate SkipAnalyzer, we focus on two types of typical and critical bugs that are targeted by static bug detection, i.e., Null Dereference and Resource Leak as subjects. We employ Infer to aid the gathering of these two bug types from 10 open-source projects. Consequently, our experiment dataset contains 222 instances of Null Dereference bugs and 46 instances of Resource Leak bugs. Our study demonstrates that SkipAnalyzer achieves remarkable performance in the mentioned static analysis tasks, including bug detection, false-positive warning removal, and bug repair. In static bug detection, SkipAnalyzer achieves accuracy values of up to 68.37% for detecting Null Dereference bugs and 76.95% for detecting Resource Leak bugs, improving the precision of the current leading bug detector, Infer, by 12.86% and 43.13%, respectively. For removing false-positive warnings, SkipAnalyzer can reach a precision of up to 93.88% for Null Dereference bugs and 63.33% for Resource Leak bugs. Additionally, SkipAnalyzer surpasses state-of-the-art false-positive warning removal tools. Furthermore, in bug repair, SkipAnalyzer can generate syntactically correct patches to fix its detected bugs with a success rate of up to 97.30%.

==> figure/RQ1-nd-bad.tex <==
\begin{figure}[h]
\begin{center}
    
\begin{lstlisting}[escapechar=!, escapeinside={(*@}{@*)}]
public IView.Label view(D source) {
        return Objects.nonNull(this.view) ? this.view.toActionView(source) : null;
}

\end{lstlisting}

\fbox{
    \begin{minipage}{8.5cm}
        \textbf{Warning:} The object this.view could potentially be null and dereferenced later.
    \end{minipage}
}
    
\end{center}

\caption{An example of an erroneously detected Null Dereference bug by SkipAnalyzer. In this instance, it is apparent that the object "this.view" undergoes a null value check, and, as a result, it does not represent a null dereference bug.}
\label{fig:rq1-ex-nd-bad}
\end{figure}



==> figure/RQ1-nd-good.tex <==
\begin{figure}[h]
\begin{center}
    
\begin{lstlisting}[escapechar=!, escapeinside={(*@}{@*)}]
public void init() {
    logger.info("python task params {}", taskRequest.getTaskParams());

    pythonParameters = JSONUtils.parseObject(taskRequest.getTaskParams(), PythonParameters.class);

    if (!pythonParameters.checkParameters()) {
        throw new TaskException("python task params is not valid");
    }
}

\end{lstlisting}

\fbox{
    \begin{minipage}{8.5cm}
        \textbf{Warning:} The objects taskRequest and pythonParameters or the results of the method calls taskRequest.getTaskParams() and pythonParameters.checkParameters() could potentially be null. However, their nullability is not checked before they are used, which could lead to a null dereference bug.
    \end{minipage}
}
    
\end{center}

\caption{An example of a detected Null Dereference bug by SkipAnalyzer}
\label{fig:rq1-ex-nd-good}
\end{figure}

==> figure/RQ1-rl-bad.tex <==
\begin{figure}[h]
\begin{center}
    
\begin{lstlisting}[escapechar=!, escapeinside={(*@}{@*)}]
private static void writeQuietly(File file, String text) {
    try {
        PrintStream out = newPrintStream(new FileOutputStream(file));
        out.println(text);
        out.close();
    } catch (IOException ignored) {
        // ignored
    }
}
\end{lstlisting}

\fbox{
    \begin{minipage}{8.5cm}
        \textbf{Warning:} The method acquires a PrintStream resource but does not release it properly. The resource is not closed in a finally block or using try-with-resources syntax, which indicates a potential resource leakage bug.
    \end{minipage}
}
    
\end{center}

\caption{An example of an erroneously detected Resource Leak bug by SkipAnalyzer. In this example, resource of type FileOutputStream has been acquired and released afterwards.}
\label{fig:rq1-ex-rl-bad}
\end{figure}



==> figure/RQ1-rl-good.tex <==
\begin{figure}[h]
\begin{center}
    
\begin{lstlisting}[escapechar=!, escapeinside={(*@}{@*)}]
protected PrintWriter createTracer() throws MojoExecutionException {
    try {
        java.nio.file.Files.createDirectories(outputDirectory.toPath());
        return newPrintWriter(new FileOutputStream(
            outputDirectory.toPath().resolve("trace.log").toFile()));
    } catch (IOException e) {
        throw new MojoExecutionException("Could not initialize trace file", e);
    }
}
\end{lstlisting}

\fbox{
    \begin{minipage}{8.5cm}
        \textbf{Warning:} Resource of type java.io.FileOutputStream acquired by call to new FileOutputStream(...) is not released afterwards.
    \end{minipage}
}
    
\end{center}

\caption{An example of a detected Resource Leak bug by SkipAnalyzer.}
\label{fig:rq1-ex-rl-good}
\end{figure}



==> figure/RQ2-nd-bad.tex <==
\begin{figure}[h]
\begin{center}
    
\begin{lstlisting}[escapechar=!, escapeinside={(*@}{@*)}]
public IView.Label view(D source) {
    return Objects.nonNull(this.view) ? this.view.toActionView(source) : null;
}
\end{lstlisting}

\fbox{
    \begin{minipage}{8.5cm}
        \textbf{Warning:} object `Action.view` last accessed on line 74 could be null and is dereferenced at line 74.
    \end{minipage}
    
}
\fbox{
    \begin{minipage}{8.5cm}
        \textbf{Tool:} The warning is correct. The reported case is a potential null dereference bug.
    \end{minipage}
}
    
\end{center}

\caption{SkipAnalyzer failed to detect a false-positive warning in the given example for a Null Dereference bug.}
\label{fig:rq2-ex-nd-bad}
\end{figure}



==> figure/RQ2-nd-good.tex <==
\begin{figure}[h]
\begin{center}
    
\begin{lstlisting}[escapechar=!, escapeinside={(*@}{@*)}]
public String decorateValue(@Nonnull Object p, @Nullable Supplier<String> dft) {
    String result = IAzureMessage.super.decorateValue(p, null);
    if (Objects.isNull(result) && Objects.nonNull(this.valueDecorator)) {
        result = this.valueDecorator.decorateValue(p, this);
    }
    return Objects.isNull(result) && Objects.nonNull(dft) ? dft.get() : result;
}
\end{lstlisting}

\fbox{
    \begin{minipage}{8.5cm}
        \textbf{Warning:} object `dft` could be null and is dereferenced later.
    \end{minipage}
    
}
\fbox{
    \begin{minipage}{8.5cm}
        \textbf{Tool:} The warning is a false-positive. In the provided Java code, the object `dft` is checked for null before it's used (dereferenced). The ternary operator `$?$` ensures that `dft.get()` is only called if `dft` is not null. Therefore, there is no potential null dereference issue with `dft`.
    \end{minipage}
}
    
\end{center}

\caption{An example of a detected false-positive warning by SkipAnalyzer for a Null Dereference bug.}
\label{fig:rq2-ex-nd-good}
\end{figure}



==> figure/RQ2-rl-bad.tex <==
\begin{figure}[h]
\begin{center}
    
\begin{lstlisting}[escapechar=!, escapeinside={(*@}{@*)}]
protected boolean confirm(List<AzureTask<?>> tasks) throws MojoFailureException {
    try {
        final IPrompter prompter = new DefaultPrompter();
        System.out.println(CONFIRM_PROMPT_START);
        tasks.stream().filter(t -> StringUtils.isNotBlank(t.getTitle().toString())).forEach((t) -> System.out.printf("\t- %s%n", t.getTitle()));
        return prompter.promoteYesNo(CONFIRM_PROMPT_CONFIRM, true, true);
    } catch (IOException e) {
        throw new MojoFailureException(e.getMessage(), e);
    }
}
\end{lstlisting}

\fbox{
    \begin{minipage}{8.5cm}
        \textbf{Warning:} resource of type \\
        `com.microsoft.azure.maven.prompt.DefaultPrompter` acquired by call to `new()` at line 83 is not released after line 86.
    \end{minipage}
    
}
\fbox{
    \begin{minipage}{8.5cm}
        \textbf{Tool:} The warning is incorrect. The resource `DefaultPrompter` does not need to be released as it does not hold any system resources that need explicit release.
    \end{minipage}
}
    
\end{center}

\caption{SkipAnalyzer wrongly detected a warning as false-positive in the given example for a Resource Leak bug.}
\label{fig:rq2-ex-rl-bad}
\end{figure}



==> figure/RQ2-rl-good.tex <==
\begin{figure}[h]
\begin{center}
    
\begin{lstlisting}[escapechar=!, escapeinside={(*@}{@*)}]
public synchronized Properties loadMeta() throws Exception {
    File metaFile = new File(META_FILE_NAME);
    if (!metaFile.exists() && !metaFile.getParentFile().mkdirs() && !metaFile.createNewFile()) {
        throw new IllegalStateException("failed to create meta file: " + metaFile.getAbsolutePath());
    }
    
    try (FileInputStream inStream = new FileInputStream(metaFile)) {
        meta.load(inStream);
    }
    return meta;
}
\end{lstlisting}

\fbox{
    \begin{minipage}{8.5cm}
        \textbf{Warning:} resource of type `java.io.FileInputStream` acquired to `inStream` by call to `FileInputStream(...)` at line 116 is not released after line 116.
    \end{minipage}
    
}
\fbox{
    \begin{minipage}{8.5cm}
        \textbf{Tool:} The warning is a false positive. The `FileInputStream` is opened within a try-with-resources statement, which ensures that the resource is closed at the end of the statement, regardless of whether the try block completes normally or abruptly due to an exception. Therefore, there is no resource leakage in this code.
    \end{minipage}
}
    
\end{center}

\caption{An example of a detected false-positive warning by SkipAnalyzer for a Resource Leak bug.}
\label{fig:rq2-ex-rl-good}
\end{figure}



==> figure/discussion/ND2.tex <==
\begin{figure}[h]
\begin{center}
    
\begin{lstlisting}[escapechar=!, escapeinside={(*@}{@*)}]
public synchronized boolean hasInitialDeviceList() {
    checkState(state.equals(State.INITIALIZED), "Android Debug Bridge is not initialized.");
    return adb.hasInitialDeviceList();
  }
\end{lstlisting}

\fbox{
    \begin{minipage}{8.5cm}
        \textbf{Ground Truth Warning:} object ``adb'' last accessed on line 120 could be null and is dereferenced at line 120.
    \end{minipage}
}

\fbox{
    \begin{minipage}{8.5cm}
        \textbf{{\tool}'s Explanation:} The code checks if the ``state'' object is equal to ``State.INITIALIZED'' before calling the ``hasInitialDeviceList()'' method on the ``adb'' object. Therefore, there is no potential null dereference bug in this code.
    \end{minipage}
}

\end{center}

\caption{An example of a missing \textit{Null Dereference} bug by SkipAnalyzer. In this particular case, the ``adb'' object is declared as an instance variable outside of the method where the \textit{Null Dereference} is detected. Consequently, our tool attempts to establish a connection between the state check in the preceding line and the \textit{Null Dereference} issue, even though the two lines may not be directly related. }
\label{fig:discussion-nd2}
\end{figure}



==> results/RQ1.tex <==
\begin{figure*}[t!]
\begin{center}
    
\includegraphics[width=\textwidth]{results/RQ1-results-600.png}
    
\end{center}

\caption{Summary of results for Static Bug Detection (RQ1). In this figure, "ND" stands for "Null Dereference" and "RL" stands for "Resource Leak".}
\label{fig:rq1-results}
\end{figure*}



==> table/RQ2-skip.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[t]
\caption{Summary of {\tool}'s results in False-Positive Warning Removal (RQ2) on warnings generated in Sec. \ref{sec:rq1}. In this table, \textbf{$\text{P}_{\text{Original}}$} is the precision of SkipAnalyzer for the corresponding bug type and \textbf{$\text{P}_{\text{After}}$} is the precision of SkipAnalyzer after applying False-Positive Warning Removal process using the corresponding strategy and model. ``Imp.'' indicates the amount of precision improvement. In this table, rows highlighted in \tikzcircle[yellow, fill=yellow]{2pt} indicate the best combination of model and strategy for \textit{Null Dereference} bugs. Also, the records that have no improvement in precision are shown with ``--''.}
\label{table:rq2-skip-warnings}
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\textbf{Bug Type} &
  \textbf{Strategy} &
  \textbf{Model} &
  \textbf{$\text{P}_{\text{Original}}$} &
  \textbf{$\text{P}_{\text{After}}$} &
  \textbf{Imp.} &
  \textbf{Recall} &
  \textbf{Accuracy} &
  \textbf{F1-Score} \\ \hline
 &                             & GPT-3.5-Turbo & \cellcolor[HTML]{FFFFC7} & 70    & -               & 19.27 & 32.93 & 30.22 \\ \cline{3-3} \cline{5-9} 
 & \multirow{-2}{*}{Zero Shot} & GPT-4         & \cellcolor[HTML]{FFFFC7} & 86    & \textbf{+4.13}  & 26.72 & 37.45 & 40.78 \\ \cline{2-3} \cline{5-9} 
 &                             & GPT-3.5-Turbo & \cellcolor[HTML]{FFFFC7} & 67    & -               & 30.72 & 32.72 & 42.26 \\ \cline{3-3} \cline{5-9} 
 & \multirow{-2}{*}{One Shot}  & GPT-4         & \cellcolor[HTML]{FFFFC7} & 97.5  & \textbf{+15.63} & 52.72 & 59.92 & 68.44 \\ \cline{2-3} \cline{5-9} 
 & \cellcolor[HTML]{FFFFC7}    & GPT-3.5-Turbo & \cellcolor[HTML]{FFFFC7} & 73.97 & -               & 38.18 & 38.90 & 50.36 \\ \cline{3-3} \cline{5-9} 
\multirow{-6}{*}{Null Dereference} &
  \multirow{-2}{*}{\cellcolor[HTML]{FFFFC7}Few Shot} &
  \cellcolor[HTML]{FFFFC7}GPT-4 &
  \multirow{-6}{*}{\cellcolor[HTML]{FFFFC7}81.87} &
  \cellcolor[HTML]{FFFFC7}98.18 &
  \cellcolor[HTML]{FFFFC7}\textbf{+16.31} &
  \cellcolor[HTML]{FFFFC7}77.45 &
  \cellcolor[HTML]{FFFFC7}80.25 &
  \cellcolor[HTML]{FFFFC7}\textbf{86.59}
\end{tabular}
\end{table*}

==> table/infer-result.tex <==
\begin{table}[t!]
\caption{Performance of Infer in static bug detection. ``Total'' indicates the total number of warnings, ``TP'' indicates the number of true-positive warnings, ``FP'' indicates the number of false-positive warnings. 
%\song{learn how to indicate parenthesis in latex, it's not simply ""}\mamad{done. thanks for clarification.}
}
\label{table:infer-results}
\centering
\resizebox{0.5\textwidth}{!}{
    \begin{tabular}{c|c|ccc|c}
    \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Bug Type}} & \multicolumn{3}{c|}{\textbf{Infer Results}}                                          & \multirow{2}{*}{\textbf{Precision}} \\ \cline{3-5}
                                      &                                    & \multicolumn{1}{c|}{\textbf{Total}} & \multicolumn{1}{c|}{\textbf{TP}} & \textbf{FP} &                                     \\ \hline
    \multirow{2}{*}{Our collection}   & Null Dereference                   & \multicolumn{1}{c|}{436}            & \multicolumn{1}{c|}{222}         & 214         & 50.9\%                              \\ \cline{2-6} 
                                      & Resource Leak                      & \multicolumn{1}{c|}{116}            & \multicolumn{1}{c|}{46}          & 70          & 39.6\%                              \\ \hhline{======}
    \multirow{2}{*}{Projects from~\cite{kharkar2022learning}}     & Null Dereference                   & \multicolumn{1}{c|}{95}             & \multicolumn{1}{c|}{62}          & 33          & 65.2\%                              \\ \cline{2-6} 
                                      & Resource Leak                      & \multicolumn{1}{c|}{13}             & \multicolumn{1}{c|}{7}           & 6           & 53.8\%                             
    \end{tabular}
}
\end{table}
